Learning to Group: A Bottom-Up Framework for 3D Part Discovery in Unseen Categories

We address the problem of discovering 3D parts for objects in unseen categories. Being able to learn the geometry prior of parts and transfer this prior to unseen categories pose fundamental challenges on data-driven shape segmentation approaches. Formulated as a contextual bandit problem, we propose a learning-based agglomerative clustering framework which learns a grouping policy to progressively group small part proposals into bigger ones in a bottom-up fashion. At the core of our approach is to restrict the local context for extracting part-level features, which encourages the generalizability to unseen categories. On the large-scale fine-grained 3D part dataset, PartNet, we demonstrate that our method can transfer knowledge of parts learned from 3 training categories to 21 unseen testing categories without seeing any annotated samples. Quantitative comparisons against four shape segmentation baselines shows that our approach achieve the state-of-the-art performance.

==> tex/exp_tb0.tex <==
\begin{table}[h]
\centering
\begin{tabular}{| m | c | c | c | c | c | c | c | c |c |c | c | c | c |}
% \hline
% ~
% & \multicolumn{11}{c|}{Novel Category}
% \\
\hline
 ~ 
 & \includegraphics[width=0.45cm]{./fig/cat_icon/bag.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/bed.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/bottle.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/bowl.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/clock.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/dishwasher.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/display.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/door.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/earphones.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/faucet.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/hat.png}
 \\
 \hline
	
PartNet & 18.2 &	9.7&	40.7&	73.5&	30.3&	30.4&	43.6&	32.1&	16.5 &	16.6 &52.5\\	
 \hline

SGPN & 21.4 &	7&	46.7&	53.3&	27.7&	8.7& 34.8& 28.9& 25.5&	20&	37\\
 \hline

GSPN & 34.4 &	8.4&	46.9&	72.8&	42.3&	\textbf{40.6}&	57.8&	37.4&	28.4&	25.3	&31.7	\\
 \hline

WCSeg & \textbf{43.1} &	8.7 &	\textbf{59.1} &69.8 &	38.7 &	27.5 &	61.1 & 32.3  &  \textbf{38}&	\textbf{47.8} &	\textbf{53.4} \\ 	
 \hline

Ours & 41.5 & \textbf{11.3} & 49.3 & \textbf{75.7} & \textbf{43.8} & 31 & \textbf{66.7} & \textbf{38.2} & 34.4 & 32.3 & 40
 \\	
 \hline
%  ~ & \multicolumn{10}{c|}{Novel Category} & ~  \\
 \hline
  

 & \includegraphics[width=0.45cm]{./fig/cat_icon/keyboard.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/knife.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/laptop.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/microwave.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/mug.png}
 & \includegraphics[width=0.45cm]{./fig/cat_icon/refrigerator.png}
  & \includegraphics[width=0.45cm]{./fig/cat_icon/scissors.png}
  & \includegraphics[width=0.45cm]{./fig/cat_icon/table.png}
  & \includegraphics[width=0.45cm]{./fig/cat_icon/trashcan.png}
  & \includegraphics[width=0.45cm]{./fig/cat_icon/vase.png}
  & UAvg.
  \\
  \hline

PartNet  &	0.4&	33.6&	82.1&	29.6&	33&	25&	0.8&	38.9&	13.6&	36.8&	35.7\\
 \hline

SGPN &	0.4&	31&	67.3&	7.2&	13.3&	5.9&	6.4&	34.8&	7.75&	27.5&	30.8\\
 \hline

GSPN &0.4	&18.9	&92.9	&\textbf{39.2}	&40.6	&26.4&	3.7	&34.6&	12.7&	41.4&	34.7\\
 \hline

WCSeg &	0.3 &	\textbf{62.4} &	62.1 &	30 &	52.6 &	19.9 &	\textbf{46.3} &	30.2 &	13.2 & 33 &	33\\
 \hline

Ours &	0.4 & 46.6 & \textbf{96.9} & 35.9 & \textbf{53.3} & \textbf{27.6} & 16.7 & \textbf{45} & \textbf{15.2} & \textbf{43.4} & \textbf{42.9}
 \\
 \hline
\end{tabular}
\caption{Quantitative Evaluation on unseen categories. %Algorithm P, S, G, W, O refer to PartNet-InsSeg, SGPN, GSPN, WCSeg and Ours, respectively. 
The number is the average among mean recall of three levels segmentation results in PartNet. UAvg. is average among unseen categories over shape numbers.}
\label{tab:main}
\end{table}

==> tex/fig_policy.tex <==
\begin{figure}[h]
    \centering

\includegraphics[width=0.47\textwidth]{fig_policy/1_greedy.png}
\includegraphics[width=0.47\textwidth]{fig_policy/1.png}
\includegraphics[width=0.47\textwidth]{fig_policy/4_greedy.png}
\includegraphics[width=0.47\textwidth]{fig_policy/4.png}
\includegraphics[width=0.47\textwidth]{fig_policy/7_greedy.png}
\includegraphics[width=0.47\textwidth]{fig_policy/7.png}
\includegraphics[width=0.47\textwidth]{fig_policy/6_greedy.png}
\includegraphics[width=0.47\textwidth]{fig_policy/6.png}
\includegraphics[width=0.47\textwidth]{fig_policy/24_greedy.png}
\includegraphics[width=0.47\textwidth]{fig_policy/24.png}
 \subfigure[w/o the rectification module]{\includegraphics[width=0.47\textwidth]{fig_policy/6_greedy.png}}
 \subfigure[w/ the rectification module]{\includegraphics[width=0.47\textwidth]{fig_policy/6.png}}
\caption{Qualitative results. Figures show the changes of the relative size of a pair of sub-parts during the grouping process. The X-axis is the iteration number and Y-axis is the relative size defined in Appendix~\ref{section: rectification visualization}. Each row represents the grouping process for the same shape. The left column is the results without the rectification module.}
\label{fig:policy size plot}
\end{figure}


==> tex/intro_backup.tex <==
\begin{figure}[!htp]
    \centering
    \includegraphics[width=1.\textwidth]{fig/intro.png}
    \caption{Our Grouping Algorithm.}
    \label{fig:intro}
\end{figure}

\section{Introduction}
\label{sec:intro}

\hza{Tasks and motivation} We know that airplane, car and bicycles can run on earth at the first glance as they all share circle-like wheels. Such part-level information lies the foundation for perception and reasoning about the new shape, which results in decomposing/segmenting an new shape into parts an crucial task in 3D computer vision. [EMPHASIS: this problem is more reasonable in 3D.]

\hza{Related Work} Extensive research have been done in 3d mesh segmentation. These methods typically fall into two categories: learning-based and geometry-based. The learning based methods such as \cite{sgpn, yi2019gspn, mo2019partnet} usually fuse whole shape's information to generate part proposals with neural network but can hardly generalize to new categories.

\hza{History} Geometry-based methods only utilize local features at every region of the shape and grouping them by a clustering algorithm~[CITE]. Such methods can work well on new categories. However, without of the information driven by data, the methods' performance highly rely on human experts' knowledge.

\hza{Method: brief introduction} We emphasis the importance of the idea of geometry-based methods that making decision locally is very important for zero-short learning. To achieve this, we propose an iteratively grouping method to combine the advantage of both learning-based and geometry-based methods. Our method runs in a bottom-up way, starting from a set of sub-part proposal and gradually merge the sub-parts into one, as illustrate in [Figure]. Borrowing idea from Reinforcement Learning, we formalize the process as a Markov Decision Process and train a [emphasis: local] merge policy to merge the sub-parts. Celebrated PartNet dataset~[CITE] provide a rich reward so that we can supervise the process efficiently.

\hza{Method: Significance} Our method has several benefits. First, we use only local information to group the part, which enables generalization on new category if the local properties are known. But as the grouping process continue and the sub-part size increasing, the sub-parts will tend to look like a part and thus our methods will utilize high-level and more global subpart information to make reasonable grouping decision, which guarantees the accuracy.
Our method is significantly different to previous methods as we don't simply run a neural network once to get the perception results, but model the grouping process as a multi-step decision making problem. %[Too vague] In this way, we simulate the human's thinking process: put attention to one point of the shape, go around and gradually find the remaining part. We believe that modeling the learning task as a stochastic process will bridge the gap between the perception and reasoning. The experiments on several dataset demonstrate the superiority of our method.
\hza{WORDS FOR REMAINING CONTRIBUTIONS}

%2. Learning provides feedback to guide the process; 3. Generalize clustering towards a search process; (automatically part hierarchy.

\hza{Contributions} Our contributions are
\begin{itemize}
    \item We have proved that context-free is important for generalization and plays a crucial role in zero-shot learning.
    \item Our bottom-up grouping method builds a intermediate semi-part representation with rich semantic meanings.
    \item We modeled the grouping process as a sequential decision process and showed that an RL-like policy can improve performance and capture semantic meaningful information.
    \item We quantitatively evaluated our methods on proposed metrics for new categories and achieved surprising generalization results. 
\end{itemize}
